Quantum information measures and their applications in quantum field theory

In the last decades, it has been understood that a wide variety of phenomena in quantum field theory (QFT) can be characterised using quantum information measures, such as the entanglement entropy of a state and the relative entropy between quantum states in the same Hilbert space. In this thesis, we use these and other tools from quantum information theory to study several interesting problems in quantum field theory. The topics analysed range from the study of the Aharonov-Bohm effect in QFT using entanglement entropy, to the consistence of the Ryu-Takayanagi formula (proposed in the context of the AdS/CFT duality) using properties of relative entropy. We show that relative entropy can also be used to obtain new interesting quantum energy inequalities, that constrain the spatial distribution of negative energy density.

==> ap1.tex <==
\chapter{\label{ch:ap1}Apendice: Medidas de entrelazamiento}

Cosas que eventualmente podrían ir acá:\\
\\
- Rol de la entropía en la teoría de la información.

==> campos.tex <==
\section{Entropía en teoría de campos}

El estado relevante para el cálculo de valores de expectación de observables en una región $V$ es el operador densidad reducido $\rho_V$. A partir del operador densidad reducido es posible evaluar la entropía de entrelazamiento en la región, definida a partir de la ecuación (\ref{neumann}) para el estado de vacío (cuando el estado global es el vacío, se la suele llamar \textbf{entropía geométrica}).

Al considerar teorías relativistas, la entropía geométrica resulta ser divergente \cite{bombelli,hooft}. Estas divergencias se pueden entender como consecuencia del entrelazamiento presente en las fluctuaciones del vacío alrededor de la frontera de $V$ (ver figura \ref{fluctuaciones}). El proceso de localización conlleva inevitablemente a la creación de pares de partícula-antipartícula. Si una de las partículas se encuentra dentro de $V$ y la otra fuera, para hallar el operador densidad reducido $\rho_V$, la partícula dentro de $V$ queda como una partícula real mientras los grados de libertad asociados a la otra se trazan.
\begin{figure}[h]
\begin{center}
\includegraphics[width=5cm]{fluctuaciones.jpg}
\end{center}
\caption{\textbf{Fluctuaciones del vacío}. El proceso de localización en teorías relativistas lleva a la creación de pares de partícula-antipartícula. El entrelazamiento en estos pares es la causa de las contribuciones divergentes a la entropía geométrica.} \label{fluctuaciones}
\end{figure}

Dada la naturaleza ultravioleta del problema, los términos divergentes aparecen en el cálculo de la entropía de entrelazamiento también para los estados excitados de energía finita reducidos a la región $V$.

En esta sección presentamos una introducción general al cálculo de entropía en teoría de campos. También desarrollamos sobre algunas de las aplicaciones de esta cantidad y sus conexiones con diversos e interesantes problemas.

\subsection{Estructura de divergencias para la entropía en teoría de campos}

Como comentamos anteriormente, el problema que se plantea es calcular la entropía de entrelazamiento en una región del espacio, para una teoría de campos. Una forma de entender a la teoría de campos es pensando primero en una teoría con un número discreto de grados de libertad y tomando luego el límite al continuo.

\begin{figure}[h]
\begin{center}
\includegraphics[width=7cm]{red1.jpg}
\end{center}
\caption{\textbf{COMPLETAR.} COMPLETAR.} \label{red1}
\end{figure}
En la figura \ref{red1} representamos una región del espacio dividida en dos partes: un círculo $A$ y su complemento $B$. Los puntos representan una red que discretiza el espacio. El espacio de Hilbert de nuestro sistema estará compuesto por dos partes $\cal{H} = \cal{H}_A \otimes \cal{H}_B $; supongamos que nos interesa estudiar la entropía para la región $A$, para un estado global $\rho$. Por lo comentado en el capítulo anterior, sabemos que el estado relevante para hacer este cálculo está dado por el operador densidad reducido $\rho_A=\tr_B \rho$, y que la entropía es la entropía de von Neumann para $\rho_A$: $S_A=-\tr \left(\rho_A \log \rho_A\right)$. Esta entropía se reduce a la entropía termodinámica cuando el estado es térmico.

Cuando el estado no es térmico aparecen otras contribuciones. Para ver estas contribuciones presentamos el siguiente ejemplo.

\subsubsection{Un primer ejemplo}
Consideremos como ejemplo el caso de una teoría escalar libre no masiva en dos dimensiones espaciales (siguiendo a \textbf{[SREDNICKI 1993]}). Discretizando el espacio como en la figura \ref{red2} obtenemos una teoría en la red
\begin{eqnarray}
H &=&\frac{1}{2} \int d^2 x \left[ \dot{\phi}\left( x\right)^2+\left( \nabla\phi\left(x\right) \right)^2 \right] \longrightarrow \nonumber \\ 
\longrightarrow H &=& \frac{1}{2} \sum \epsilon ^2 \left[\dot{\phi}_i^2 + \sum \frac{\left(\phi_i-\phi_j\right)^2}{\epsilon ^2} \right]\,,
\end{eqnarray}
donde $\epsilon$ es la distancia entre dos primeros vecinos en la red.

\begin{figure}[h]
\begin{center}
\includegraphics[width=7cm]{red2.jpg}
\end{center}
\caption{\textbf{COMPLETAR.} COMPLETAR.} \label{red2}
\end{figure}
Elegimos a $\rho$ como el estado de vacío (estado fundamental en la teoría en la red) para hacer el cálculo de entropía geométrica en la región cuadrada de lado $L$ de la figura \ref{red2}. Esta cuenta puede hacerse numéricamente y se obtiene \textbf{CITA}
\begin{equation}
S=0.075 \frac{4L}{\epsilon}-0.047 \log\left(\frac{L}{\epsilon}\right)+cte = 0.075 \frac{\cal{A}}{\epsilon}-0.047 \log\left(\frac{L}{\epsilon}\right)+cte\,,\label{unaecmas}
\end{equation}
donde llamamos $\cal{A}$ al perímetro del cuadrado.

El término proporcional al perímetro se conoce como \textbf{término de área}, dado que es un término proporcional al área del borde de la región (recordar que en este caso las regiones son figuras en dimensión espacial $2$, por lo que el perímetro de la región es el área del borde de la región).  También vemos que hay una contribución logarítmica que, al igual que el término de área, diverge en el límite $\epsilon \longrightarrow 0$. Estas son el tipo de divergencias ultravioletas de las que hablamos al comienzo de este capítulo.

\begin{figure}[h]
\begin{center}
\includegraphics[width=7cm]{red3.jpg}
\end{center}
\caption{\textbf{COMPLETAR.} COMPLETAR.} \label{red3}
\end{figure}
Consideremos ahora la región marcada en la figura \ref{red3}, de igual perímetro que la anterior, pero diferente geometría. El cálculo para la entropía de esta región arroja el siguiente resultado
\begin{equation}
S = 0.075 \frac{\cal{A}}{\epsilon}- \frac{6}{4} 0.047\log\left(\frac{L}{\epsilon}\right)+cte\,,
\end{equation}
es decir, tenemos el mismo término de área y además vemos que el coeficiente del término logarítmico aumenta. De hecho, el coeficiente del término logarítmico aumenta con el número de vértices \textbf{REFERENCIA}) y en general se tiene
\begin{equation}
S = c_1 \frac{\cal{A}}{\epsilon}-\sum_{vert.} c_{\log}\left(\theta\right) \log\left(\frac{L}{\epsilon}\right)\,.
\end{equation}

\begin{figure}[h]
\begin{center}
\includegraphics[width=7cm]{red4.jpg}
\end{center}
\caption{\textbf{COMPLETAR.} COMPLETAR.} \label{red4}
\end{figure}
Hasta aquí pareciera apreciarse cierta regularidad en el coeficiente del término de área; sin embargo, si tomamos una región como la diagramada en la figura \ref{red4} (es decir, también un cuadrado de lado $L$ pero rotado respecto al de la figura \ref{red2}, obtenemos
\begin{equation}
S = 0.085 \frac{\cal{A}}{\epsilon}- 0.047 \log\left(\frac{L}{\epsilon}\right)+cte\,.
\end{equation}
Esto nos demuestra que el término de área no tiene la simetría rotacional que debería tener en la teoría del continuo. El punto interesante es que el coeficiente del término logarítmico es igual al dado por la ecuación \reef{unaecmas}, lo que indica que no siente los efectos producidos por cambiar la forma de la red. En este sentido, diremos que el término logarítmico es un término universal, que se espera que contenga información relevante de la teoría de campos.

Con este ejemplo sencillo confirmamos el hecho de que la entropía para una región es divergente en la teoría de campos. Además, vimos que en general los términos divergentes no son universales (a excepción del término logarítmico). Esta universalidad del término logarítmico también se confirma con el resultado para la entropía en teorías conformes en $1+1$ dimensiones \textbf{REFERENCIA}
\begin{equation}
S\left(r\right)=\frac{c}{3}\log\left(\frac{r}{\epsilon}\right)+c_0\,,
\end{equation}
siendo $c$ la carga central de Virasoro de la teoría.

\subsubsection{Intervalo en 1+1 para el campo de Dirac a T$\neq$0}

Otro ejemplo interesante, para visualizar el rol de los términos divergentes y finitos en la entropía, es el del cálculo de la entropía de un intervalo espacial en una teoría de Dirac no masiva en $1+1$ dimensiones a temperatura $T$. En este caso, la entropía resulta\cite{cardy}
\begin{equation}\label{tfinita}
S=\frac{1}{3}\ln\left[\frac{1}{\pi \epsilon T}\textrm{sinh}\left(\pi L T\right)\right]\,,
\end{equation}
donde $\epsilon$ es un cutoff ultravioleta con unidades de distancia. En el límite en que $L T\rightarrow \infty$, la ecuación (\ref{tfinita}) da
\begin{equation}\label{finnn}
S\approx\frac{1}{3}\ln(\epsilon)+\ln\left(\frac{1}{T}\right)+\frac{\pi}{3}L T\,,
\end{equation}
donde el último sumando de \reef{finnn} dice que la entropía crece en forma proporcional al volumen, como suele ocurrir para un estado térmico. Para $L T\rightarrow 0$ se obtiene
\begin{equation}
S\approx-\frac{1}{3}\ln\left(\frac{L}{\epsilon}\right)\,,
\end{equation}
que es un resultado que también puede obtenerse independientemente utilizando el formalismo de tiempo real, para la misma teoría con temperatura nula (este cálculo, utilizando el formalismo de tiempo real se puede ver por ejemplo en \textbf{REFERENCIA}). El término $\frac{\pi}{3}L T$ se obtendría también si uno pusiera al sistema en una caja con condiciones de borde a temperatura $T$, tomando el límite de $L$ grande. De (\ref{finnn}), se ve que en este límite, es posible separar el término proporcional al volumen de la parte divergente. Se dice entonces que este término es universal, o sea, independiente del \textit{cutoff} o las condiciones de borde que se impongan en la caja. \textbf{VER ESTO}

\subsubsection{Estructura de divergencias y términos universales}

En $d$ dimensiones espaciales, para cualquier teoría de campos se tiene \textbf{REFERENCIA}
\begin{equation}\label{ultimaec}
S(V)=g_{d-1}[\partial V]\epsilon^{-(d-1)}+...+g_1 [\partial V]\epsilon^{-1}+g_0[\partial V]\ln(\epsilon)+S_0(V)\,,
\end{equation}
siendo $S_0(V)$ una contribución finita, $\epsilon$ un \textit{cutoff} ultravioleta (proveniente por ejemplo de la discretización realizada para llevar la teoría de campos a la red) y cada $g_i$ una función local extensiva en el borde $\partial V$~\footnote{Esto está asociado a que los modos de corta longitud de onda que se encuentran entrelazados entre la región exterior y la interior a $V$ sólo pueden contribuir sobre el borde y de manera local, es decir como una integral sobre el borde.}.

El coeficiente del primer término $g_{d-1}[\partial V]$ se conoce cómo término de área. Principalmente en relación a la entropía de un agujero negro se suele decir que la entropía satisface una \textit{ley de área} $ S \sim \frac{R^{d-2}}{\epsilon^{d-2}}$ \textbf{REFERENCIAS}. Es importante remarcar que (a pesar de que resulta evidente después del ejemplo presentado en la sección anterior) esta ley de área no es una propiedad de la teoría del continuo. En la sección \ref{bhyarea} comentaremos con más detalle la relación entre la entropía de entrelazamiento y la de los agujeros negros.

Los términos proporcionales a $g_i$ para $i>0$ no tienen una interpretación física en teoría de campos, dado que no están asociados a cantidades independientes de la discretización a partir de la cual se interpreta a la teoría de campos. Sin embargo, el coeficiente $g_0$ del término logarítmico sí es universal.

\begin{figure}[h]
\begin{center}
\includegraphics[width=7cm]{red5.jpg}
\end{center}
\caption{\textbf{COMPLETAR.} COMPLETAR.} \label{red5}
\end{figure}
El término finito $S_0\left(V\right)$ contiene información sobre el estado y la región. Por ejemplo, si el estado es un estado de equilibrio térmico a una temperatura $T$, se tiene $S_0\left(V\right) \sim \kappa T^{d-1} V$, que es la entropía termodinámica usual.

%Veamos que es posible extraer información no ambigüa de este término finito. Para ello, volvemos a considerar una teoría escalar libre en dos dimensiones espaciales (sobre una red cuadrada, al igual que en el ejemplo anterior), pero ahora calcularemos la entropía para una región circular de radio $R$ como la mostrada en la figura \ref{red5}. En este caso, no aparece un término logarítmico para la entropía (ya que la región no tiene vértices)
%\begin{equation}
%S\left(R\right)=c_1 R + c_0\,.
%\end{equation}
%
%Para el caso de un estado térmico, la diferente dependencia de la entropía térmica con el volumen $S_T\sim V T$ permitiría extraer este término universal de la entropía. Una situación muy diferente se da en casos en los cuales la entropía se encuentra muy diluída, como ocurre con la entropía de la radiación de Hawking en los agujeros negros. Estos son objetos relativamente fríos, que emiten radiación a una temperatura $T\sim r_S^{-1}$ (siendo $r_s$ el tamaño del agujero negro; en el capítulo \ref{ch:agujeros}, se dan más detalles acerca de los agujeros negros). La entropía emitida en este caso viene dada heurísticamente como
%\begin{equation}
%S\approx T^3\cdot V=T^3\times\textrm{área\,de\,emisión}\times\textrm{tiempo}=\frac{R_{shell}}{r_s}\,,
%\end{equation}
%que no puede separarse de los términos divergentes $S\sim\frac{R_{shell}^2}{\epsilon^2}+\frac{R_{shell}}{\epsilon}+...$. Este problema puede subsanarse utilizando alguna otra medida de información, como se verá en la siguiente sección.
\subsection{Relación con la entropía de los agujeros negros}\label{bhyarea}



\subsection{Algunos resultados en teoría de campos}

En general, el cálculo de entropía en teoría de campos es un proceso muy complicado y se cuenta con muy pocos resultados analíticos explícitos. En esta sección, enumeraremos algunos de los resultados relevantes, para comenzar a entender un poco la estructura que se espera para la entropía en teoría de campos.

\subsection{Información mutua}\label{secmutua}

Se ha comentado que la localización estricta de un estado en una región del espacio, en teorías relativitas, da lugar a la formación de pares partícula-antipartícula y que en la aparición de estos modos de alta energía se encuentra el origen de las divergencias en la entropía de entrelazamiento. Una contribución divergente similar aparecerá en cualquier cálculo de la entropía en una región separada de otra por un horizonte causal, como es el caso de los agujeros negros. Sin embargo, la noción de entrelazamiento entre dos regiones distintas puede definirse de modo preciso en teoría de campos, aún en presencia de gravitación. Las medidas de entrelazamiento entre regiones disjuntas no presentan divergencias y son, en principio, calculables en la teoría semiclásica.\\
\\
Es posible realizar una substracción en la entropía de entrelazamiento del vacío para eliminar las divergencias provenientes de las fluctuaciones del vacío. Sin embargo, no se puede simplemente llevar a cero el valor de esta entropía, dado que existen cantidades finitas universales (independientes de la regularización) que se pueden obtener a partir de ella. Una de esas cantidades es la \textbf{información mutua}

{\small
\begin{equation}\label{infomutua}
I(A,B)=S(A)+S(B)-S(A\cup B)\,,
\end{equation}}

entre dos conjuntos disjuntos (ver figura \ref{mutua}) $A$ y $B$. Nótese que los términos divergentes, que están asociados a los bordes de las regiones se sustraen en (\ref{infomutua}). En estadística, la información mutua da una medida a la información compartida por dos sistemas. La información mutua es una cantidad bien definida en teoría de campos, con el único requerimiento de que exista una separación no nula entre las regiones $A$ y $B$, y mide el grado de no extensividad que tiene la entropía $S$.\\
\\
\begin{figure}[h]
\begin{center}
\includegraphics[width=5cm]{mutua.jpg}
\end{center}
\caption{\textbf{Información mutua}. Para dos regiones $A$ y $B$ disconexas, como las que se muestra en la figura, es posible definir una cantidad universal de la que puede inferirse la entropía de entrelazamiento.} \label{mutua}
\end{figure}

Si la región $B$, por ejemplo, se extendiera a todo el espacio de modo de tender a cubrir la región $-A$, y el contorno de $B$ se aproximara al de $A$ desde afuera, se obtendría $S(A)\approx S(-B)=S(B)$ y $S(A\cup B)\approx 0$ y, entonces

\begin{equation}\label{recupera}
I(A,B)\approx 2S(A)\,.
\end{equation}

Así, la información mutua diverge del mismo modo que la entropía cuando los conjuntos se acercan uno al otro y, de algún modo, se reproducen las divergencias presentes en $S(A)$, pero ahora en forma independiente de la regularización.

\subsubsection{Propiedades de la información mutua}\label{sectripartita}

Para un sistema cuántico general, la función $I(A,B)$ es simétrica, adimensional y positiva. Si se considera un estado producto, dado por $\rho_{A\cup B}=\rho_A \otimes \rho_B$, la información mutua $I(A,B)$ se anula. Otra propiedad interesante es la de monotonía respecto al tamaño de los conjuntos

\begin{equation}\label{monoinfo}
I(A,B)\leq I(A,C)\,,\,\textrm{si}\,\,\,B\subseteq C\,.
\end{equation}

Esta propiedad, indica que la información mutua varía suavemente con el conjunto y es una consecuencia de la propiedad de subaditividad fuerte de la entropía. También se tiene la siguiente desigualdad

\begin{equation}
I(A,B)\leq 2 \,\textrm{min}(S(A),S(B))\,.
\end{equation}

También es posible definir la \textbf{información tripartita}

\begin{equation}\label{tripartita}
I(A|B,C)=I(A,B)+I(A,C)-I(A,B\cup C)\,,
\end{equation}

que mide la información compartida entre $B$ y $C$ respecto de $A$. Por la propia definición de la información mutua (\ref{infomutua}), la información tripartita tiene simetría de permutación total

{\small
\begin{eqnarray}\label{triparentro}
&&I_3(A,B,C)\equiv I(A|B,C)=\\
&&S(A\cup B\cup C)-S(A\cup B)-S(B\cup C)-S(C\cup A)+S(A)+S(B)+S(C)\,.\nonumber
\end{eqnarray}}

Así como la información mutua mide el grado de no extensividad de la entropía, la información tripartita, en virtud de la ecuación (\ref{tripartita}), mide el apartamiento de la extensividad de la información mutua. Nótese que a diferencia de $I(A,B)$, $I_3(A,B,C)$ puede ser tanto positiva o negativa, y es nula en particular cuando el estado total es puro. Sin embargo, la condición general que hace que la información mutua sea extensiva es aún desconocida.

\subsection{El método de réplicas}

En las siguientes páginas introducimos el método de réplicas, una herramienta poderosa mediante la cual se puede hallar la traza de potencias del operador densidad. Es particularmente útil para calcular las entropías de Renyi, de las cuales proviene la entropía de entrelazamiento como una continuación analítica hacia $n=1$.

\subsubsection{Entropías de Renyi}

Ciertas propiedades no perturbativas de la funcional entrop\'{\i}a hacen de la entrop\'{\i}a geom\'etrica una herramienta muy \'util en la investigaci\'on en teor\'ia de campos. En particular, la subaditividad fuerte y la geometr\'ia relativista dan lugar a un teorema C entr\'opico en dos dimensiones, similar al teorema C de Zamolodchicov. Este teorema prueba la irreversibilidad del grupo de renormalizaci\'on en dos dimensiones, y a pesar del esfuerzo de numerosos autores no se conoce a\'un una generalizaci\'on universalmente v\'alida en m\'as dimensiones. Otras medidas de informaci\'on, las denominadas entrop\'{\i}as de Renyi

\begin{equation}
S_n\left(V\right)=\frac{1}{1-n}\log tr\rho_V^n\,,
\label{renyi}
\end{equation}

se pueden escribir en t\'ermino de valores de expectaci\'on de operadores en teor\'{\i}as relativistas, y con ello podr\'{\i}an ser utilizadas para dar una descripci\'on dual de la teor\'{\i}a original.

Las entropías de Renyi también son útiles para hallar $S\left(V\right)$ como una continuación analítica de estas hacia $n=1$

\begin{equation}
-\lim_{n\longrightarrow 1}\frac{\partial}{\partial n}tr\rho_V^n=\lim_{n\longrightarrow 1}S_n\left(V\right)=S\left(V\right)\,,
\end{equation}

donde la última igualdad se obtiene utilizando la regla de L'Hôpital.

La entrop\'{\i}a geom\'etrica es hoy uno de los candidatos mas interesantes para entender el origen estad\'{i}stico de la entrop\'{i}a termodi\'amica que presentan los agujeros negros y otras interesantes aplicaciones de ella se da en desarrollos recientes a la dualidad de Maldacena (AdS/CFT), que relaciona una teor\'{\i}a de gravedad cu\'antica en espacio anti de Sitter con una teor\'{\i}a de campos conforme en el borde asint\'otico. Existe un anzats debido a Ryu y Takayanagi basado en estas ideas hologr\'aficas sobre cómo es la funci\'on entrop\'{\i}a geom\'etrica en la teor\'{\i}a conforme. El an\'alisis directo de esta cantidad en la teor\'{\i}a de campos correspondiente permitir\'{\i}a verificar esta conjetura.

Por estas y muchas otras aplicaciones, la entropía geométrica y las entropías de Renyi son cantidades cuyo estudio es relevante. En los capítulos siguientes, estudiaremos cómo hallar estas cantidades en el formalismo de tiempo euclídeo.

\subsubsection{Representación funcional del operador densidad reducido}

Consideramos un campo escalar $\hat{\phi}\left(x,t\right)$ y una base de autovectores de este operador a tiempo $t=0$: $\hat{\phi}\left(x,0\right)\left|\alpha\right\rangle=\alpha\left(x\right)\left|\alpha\right\rangle$, donde $\alpha$ es cualquier función real. Luego, el funcional de onda del vacío se escribe como \cite{pokorski}

\begin{equation}
\Phi\left(\alpha\right)=\left\langle 0\right|\left.\alpha\right\rangle=N^{-1/2}\int_{\phi\left(x,-\infty\right)=0}^{\phi\left(x,0\right)=\alpha\left(x\right)}{\textit{D}\phi\, e^{-S_E\left(\phi\right)}}\,.
\label{funcional}
\end{equation}

Para elegir el estado de vacío, la integral funcional se realiza sobre la mitad inferior del espacio (para ``suprimir'' los estados excitados) y en tiempo euclídeo. $N^{-1/2}$ es una factor de normalización. El operador densidad en esta base es $\rho\left(\alpha,\alpha '\right)=\left\langle \alpha\right|\left.0\right\rangle\left\langle 0\right|\left.\alpha '\right\rangle=\Phi\left(\alpha\right)^{\dagger}\Phi\left(\alpha '\right)$. Hallar la matriz densidad reducida a la región $V$ implica trazar sobre los grados de libertad en $-V$ (el conjunto complementario a $V$). Para realizar esto, consideramos funciones $\alpha=\beta\oplus\alpha_V$, $\alpha '=\beta\oplus\alpha'_V$, que coinciden en $-V$ (son iguales a $\beta$), y sumamos sobre todas las posibles funciones $\beta$. Utilizando la representación (\ref{funcional}), la matriz densidad reducida se obtiene tomando dos copias de la mitad del espacio, pegándolas en $-V$ y realizando la integral funcional en este nuevo espacio \cite{larsen}

\begin{equation}
\rho_V\left(\alpha_V,\alpha'_V\right)=\int{\textit{D}\beta\,\Phi\left(\beta\oplus\alpha_V\right)^{*}\Phi\left(\beta\oplus\alpha'_V\right)}=N^{-1}\int_{\phi\left(x,0^-\right)=\alpha'_V\left(x\right),\,x\,\in V}^{\phi\left(x,0^+\right)=\alpha_V\left(x\right),\,x\in V}{\textit{D}\phi\, e^{-S_E\left(\phi\right)}}\,.
\end{equation}

Los argumentos de la matriz densidad reducida son las condiciones de contorno de la integral funcional a cada lado de los cortes en $V$.



\begin{figure}[h]
	\centering
		\includegraphics{densidad.jpg}
	\caption{\textit{La integral funcional sobre la mitad inferior del espacio euclídeo nos permite obtener la funcional de onda del vacío. La matriz densidad reducida $\rho_V$ se obtiene ``pegando'' dos copias de este semiespacio a lo largo de $-V$, el conjunto complementario a $V$.}}
	\label{densidad}
\end{figure}

\subsubsection{El método de réplicas aplicado al cálculo de la entropía}

Es posible escribir las entropías de Renyi (\ref{renyi}) en esta representación funcional. Para ello, hay que tomar $n$ copias del plano euclídeo con cortes a lo largo de $V$ y pegar el lado superior de la copia $k-$ésima con el lado inferior de la copia $\left(k+1\right)-$ésima, para $k=1,\,2,\,...,\,n$ (la copia $n+1$ se identifica con la primera copia). Esto nos deja con un espacio euclídeo de la misma dimensión que el espacio original, con singularidades cónicas de ángulo $2\pi n$ localizadas en el borde $\partial V$ de $V$. Con estas consideraciones, se tiene

\begin{equation}
tr \rho_V^{n}=\frac{Z\left[n\right]}{Z\left[1\right]^n}\,,
\end{equation}

\begin{equation}
S_n\left(V\right)=\frac{\log Z\left[n\right]-n\log Z\left[1\right]}{1-n}\,,
\label{renyi2}
\end{equation}

\begin{equation}
S\left(V\right)={\lim}_{n\longrightarrow 1} \left(1-n\frac{d}{dn}\right)Z\left[n\right]
\end{equation}
donde $Z\left[n\right]$ es la integral funcional en la variedad con $n$ ``láminas'' (que llamaremos \textbf{función de partición}), y elegimos el factor de normalización $N=Z\left[1\right]$ para que se cumpla $tr\rho_V=1$. La ecuación (\ref{renyi2}) da una representación funcional de las entropías de Renyi para $n$ entero. La entropía de entrelazamiento se obtiene haciendo una continuación analítica de $S_n$ hacia $n=1$.

\begin{figure}[h]
\begin{center}
\includegraphics[width=5cm]{replicado.jpg}
\end{center}
\caption{\textit{La $tr\rho_V^n$ está dada por una integral funcional en una variedad con $n$ láminas, construída pegando el espacio euclídeo replicado con un corte $V$.}} \label{densidad}
\end{figure}

\subsubsection{Métodos para calcular la función de partición}

En general, el cálculo de la función de partición es complicado dado que aparecen involucradas variedades no triviales debido al método de réplicas. En las siguientes subsecciones presentamos muy brevemente algunos métodos existentes para hallar $Z$.

\begin{enumerate}
\item Diagonalización en el espacio replicado

Para el caso de campos libres, es posible trasladar el problema de la variedad con $n$ ``láminas'' a uno equivalente en el cual uno trata con $n$ campos libres multivaluados desacoplados. Este método se encuentra aplicado en \cite{fosco} para calcular las entropías de Renyi de un campo de Dirac libre.

\item Heat Kernel

Otra herramienta poderosa para realizar el cálculo de la función de partición, cuando la acción es cuadrática, es el método del \textit{heat kernel}. Para introducirlo, consideramos un campo escalar libre, y notamos que

\begin{equation}
W=-\log Z=\frac{1}{2}\log\det\left(M^2-\nabla^2\right)=\frac{1}{2}tr\log\left(M^2-\nabla^2\right)\,.
\label{elibre}
\end{equation}

La función de partición se reduce entonces a la función espectral de un operador diferencial. El heat kernel se define como $K\left(x,y,t\right)=\left\langle x\right|e^{t\nabla^2}\left|y\right\rangle$, y su traza se escribe como

\begin{equation}
\zeta\left(t\right)=tr e^{t\nabla^2}=\int{dx\,K\left(x,x,t\right)}\,.
\end{equation}

La ``energía libre'' $W$ puede escribirse en términos de esta función espectral como

\begin{equation}
W=-\frac{1}{2}\int_{\epsilon}^{\infty}{dt\,e^{-M^2 t}\frac{1}{t}\zeta\left(t\right)}\,,
\end{equation}
donde $\epsilon$ es un cutoff. La ventaja de esta ecuación es que, en contraste con (\ref{elibre}), está escrita como una función de la traza de un operador que satisface una ecuación del calor local

\begin{equation}
\frac{\partial K}{\partial t}=\nabla^2 K\,,\,\,\,\,\,K\left(x,y,0\right)=\delta\left(x-y\right)\,.
\end{equation}

\item Función de Green

Otra estatregia posible para hallar la función de partición consiste en estudiar la función de Green asociada $G=\left(-\nabla^2+M^2\right)^{-1}$ en la variedad asociada al problema. $Z$ y $G$ están relacionadas a través de la identidad

\begin{equation}
\frac{d}{dM^2}\log Z=-\frac{1}{2}tr G\,.
\end{equation}

Sin embargo, no existen métodos generales para hallar $G$ en este tipo de variedades con singularidades cónicas, por lo que hay que analizar caso por caso viendo si la geometría del problema ayuda a reducir la dificultad del cálculo. Este es el método que utilizaremos en la siguiente sección para realizar un cálculo sencillo de la entropía de un campo escalar libre por el método de réplicas.
\end{enumerate}

\subsubsection{Ejemplo: Campo escalar libre en $1+1$}

Consideramos el ejemplo de un campo escalar libre en dimensión $1+1$, cuya acción euclídea es

\begin{equation}
S_E=\int d^2 r \frac{1}{2}\left[\partial_\mu\phi\partial^\mu\phi+M^2\phi^2\right]\,.
\end{equation}

Pretendemos calcular la entropía para una semirrecta, es decir, $V=\left[0,\infty\right]$ (seguiremos como referencia el cálculo realizado en \cite{pasquale}). Para hallar $tr\rho_V^n$ debemos calcular la función de partición $Z[n]$ de esta teoría en una variedad con $n$ ``láminas'' conectadas por un corte. Como ya comentamos, hay diferentes maneras de calcular la función de partición; en este caso, resultará conveniente recordar su relación con la función de Green $G_n\left(\bar{r},\bar{r}'\right)$

\begin{equation}
\frac{\partial }{\partial M^2}\log Z\left[n\right]=-\frac{1}{2}\int{d^2 rG_n\left(\bar{r},\bar{r}\right)}\,.
\end{equation}

En este caso, la función de Green satisface la siguiente ecuación sobre la variedad

\begin{equation}
\left(-\bar{\nabla}_{\bar{r}}^2+M^2\right)G_n\left(\bar{r},\bar{r}'\right)=\delta^2\left(\bar{r}-\bar{r}'\right)\,,
\label{parti}
\end{equation}
y se puede obtener hallando una base de autofunciones $f_k\left(\bar{r}\right)$ del operador de Helmholtz $\left(-\bar{\nabla}_{\bar{r}}^2+M^2\right)$

\begin{equation}
G_n\left(\bar{r},\bar{r}'\right)=\sum{N_k f_k^*\left(\bar{r}\right) f_k\left(\bar{r}'\right)}\,,
\label{helm}
\end{equation}
siendo $N_k$ una constante de normalización tal que

\begin{equation}
N_m \int{d^2 r f_m\left(\bar{r}\right)f_n\left(\bar{r}\right)}=\delta_{mn}\,.
\end{equation}

Por la simetría del problema, es conveniente escribir todo en coordenadas polares

\begin{equation}
x= r\cos \theta\,,\,\,y=r\sin \theta\,.
\end{equation}

El hecho de que la variedad tenga un corte se expresa en estas coordenadas diciendo que las autofunciones tienen que tener el mismo valor para diferencias de $2\pi n$ en $\theta$

\begin{equation}
f_k\left(r,\theta\right)=f_k\left(r,\theta+2\pi n\right)\,.
\label{contorno}
\end{equation}

Proponemos una solución a la ecuación (\ref{helm}) de la forma $f\left(r,\theta\right)=A\left(r\right)B\left(\theta\right)$, de donde obtenemos la siguientes ecuaciones

\begin{equation}
-A'' r^2-A' r+C A+M^2 r^2 A=0\,\,\,\,\,y\,\,\,\,\,B''+C B=0\,.
\end{equation}

La condición (\ref{contorno}), que se traduce en que $B\left(0\right)=B\left(2\pi n\right)$, impone que $\sqrt{C}=\frac{m}{n}$, con $m\in N$. La ecuación para $A$ es una ecuación de Bessel cuyas soluciones son las funciones de Bessel de primer y segundo tipo $J_{m/n}\left(-i M r\right)$ y $Y_{m/n}\left(-i M r\right)$, respectivamente. Como queremos soluciones regulares en $r=0$, descartamos las funciones de segundo tipo. Con estas consideraciones, obtenemos finalmente

\begin{equation}
G_n\left(r,\theta,r',\theta\right)=\frac{1}{2\pi n}\sum_{k=0}^{\infty}{d_k\int_{0}^{\infty}{\lambda}\frac{J_{k/n}\left(\lambda r\right)J_{k/n}\left(\lambda r'\right)}{\lambda^2+M^2}C_k\left(\theta,\theta'\right)d\lambda}\,,
\end{equation}
donde $d_k$ es $1$ si $k=0$ y $2$ si $k>0$, y $C_k\left(\theta,\theta'\right)=\cos\left(\frac{k\theta}{n}\right)\cos\left(\frac{k\theta'}{n}\right)+\sin\left(\frac{k\theta}{n}\right)\sin\left(\frac{k\theta'}{n}\right)$.

Para hallar la función de partición usando la ecuación (\ref{parti}) nos interesa $\bar{r}=\bar{r}'$, por lo tanto, integrando la ecuación anterior en $\theta$ y $\lambda$ obtenemos

\begin{equation}
G_n\left(r\right)=G_n\left(\bar{r},\bar{r}\right)=\sum_{k=0}^{\infty}{d_k I_{k/n}\left(M r\right)K_{k/n}\left(M r\right)}\,,
\label{coin}
\end{equation}
donde $I_{k/n}$ y $K_{k/n}$ son las funciones de Bessel modificadas de primer y segundo tipo respectivamente.

La suma sobre $k$ en (\ref{coin}) es divergente y debe regularizarse. Sin embargo, si formalmente intercambiamos la integración con la suma, podemos hallar

\begin{equation}
-\frac{\partial }{\partial M^2}\log Z\left[n\right]=\frac{1}{2}\sum_{k=1}^{\infty}{d_k\int{d^2 r d_k I_{k/n}\left(M r\right)K_{k/n}\left(M r\right)}}=\frac{1}{4n M^2}\sum_{k=0}^{\infty}{d_k k}\,.
\end{equation}

Si interpretamos la última suma como $\sum_{k=1}^{\infty}{d_k k}=2\zeta\left(-1\right)=-\frac{1}{6}$ se obtiene el resultado correcto para la entropía

\begin{equation}
S\left(V\right)=-\frac{1}{6}\log\left(\frac{\epsilon}{M^{-1}}\right)\,.
\end{equation}

\subsection{Algunas aplicaciones de la entropía de entrelazamiento}

\subsubsection{Entropía de un agujero negro}

\subsubsection{Entropía de entrelazamiento como medida de información}

\subsubsection{Aplicaciones en materia condensada como parámetro de orden}

\subsubsection{Teorema c en $1+1$}

El enunciado teorema c en $1+1$ dimensiones [A. B. Zamolodchikov, Pis'ma Zh. Eksp. Teor. Fiz. 43, 565 (1986); JETP Lett. 43, 730 (1986)] puede expresarse en dos formas equivalentes:\\
\\
1. Existe una función adimensional y universal de las constantes de acoplamiento $c=c\left(\lbrace\lambda_i\rbrace\right)$, que en el espacio de las teorías de $1+1$ dimensiones no aumenta a lo largo de las trayectorias del grupo de renormalización y que es estacionaria en los puntos fijos, donde toma un valor finito proporcional a la carga central de Virasoro $C_V$.\\
\\
2. Para toda teoría en $1+1$ dimensiones existe una función adimensional y universal función de la distancia $c=c\left(r\right)$, que no aumenta ante dilataciones y toma un valor finito proporcional a la carga central de Virasoro $C_V$ en los puntos fijos.\\
\\



La demostración del teorema c en 1+1 es particularmente sencilla si se utiliza a la entropía de entrelazamiento.

\subsubsection{Dualidad AdS/CFT}


*****
Introducir el capítulo siguiente como una aplicación de la entropía en teoría de campos a los fenómenos topológicos (en particular, al efecto Aharonov-Bohm)

==> entropia.tex <==
\chapter{\label{ch:entropia}Generalidades sobre la entropía en teorías cuánticas}

%\pagecolor[cmyk]{0.06,0.006,0.02,0.01}
\begin{chapterquote}[0.75\linewidth]
\it ''If someone points out to you that your pet theory of the universe is in disagreement with Maxwell's equations - then so much worse for Maxwell equations. If it is found to be contradicted by observation - well these experimentalists do bungle things sometimes. But if your theory is found to be against the second law of Thermodynamics, I can give you no hope; there is nothing for it but to collapse in deepest humiliation.''\\
\emph{\textbf{Sir Arthur Stanley Eddington}\\The Nature of the Physical World (1928), 74.}
\end{chapterquote}

El concepto de entropía fue introducido por R. Clausius en 1865 al estudiar sistemas termodinámicos. Sin embargo, el entendimiento moderno de la entropía como la cantidad que conecta las interpretaciones microscópica y macroscópica de un sistema es debido principalmente a L. Boltzmann y J. Gibbs. La entropía estadística de un sistema termodinámico se define como

\begin{equation}\label{ent-est}
S=k_B \ln(\Omega)\,,
\end{equation}
\\

donde $k_B=1.38066×10^{-23} J K^{-1}$ es la constante de Boltzmann y $\Omega$ es el número de microestados posibles para un dado macroestado. El número $\Omega$ es interpretado como el ''grado de desorden'' que hay en el sistema, ya que en general para un dado estado macroscópico el sistema podrá adoptar diferentes configuraciones microscópicas.\\
\\
En mecánica estadística clásica, el número de microestados de un sistema es infinito, dado que las variables que se utilizan para describir a los sistemas clásicos son continuas. Para poder contar el número de microestados en mecánica clásica, se suele realizar una \emph{discretización} en el espacio de fases, definiendo una ''celda unidad'' en forma arbitraria. El número de microestados se define entonces como el cociente entre el volumen accesible del espacio de fases y el volumen de la celda unidad. Nótese que dada la arbitrariedad en la definición de la celda unidad, la entropía queda definida a menos de una constante. Estas ambigüedades pueden ser resueltas dando una definición de entropía en mecánica cuántica.

\section{Entropía en mecánica cuántica}

En mecánica cuántica uno trata con \emph{observables} y con \emph{estados}. Los observables, como el momento, la posición, etc., se describen matemáticamente por operadores autoadjuntos en un espacio de Hilbert. La entropía no es un observable (es decir, no existe un operador con la propiedad de que su valor de expectación en algún estado sea la entropía) sino que es una función del estado. Los estados en mecánica cuántica se caracterizan en forma general por el llamado \emph{operador densidad}.

\subsection{Operador densidad}\index{subject}{Operador densidad}

El estado de un sistema cuántico se conoce completamente si se puede representar mediante un cierto vector $\left|\psi\right\rangle$ en el espacio de Hilbert. Si la información que se posee acerca del sistema es incompleta, el estado del mismo no puede representarse por un vector único sino por una mezcla estadística de vectores $\left|\psi_1\right\rangle$, $\left|\psi_2\right\rangle$,..., $\left|\psi_n\right\rangle$ y decimos que el sistema tiene probalidades $p_1$, $p_2$,..., $p_n$ ($p_i\geq0$) de encontrarse en alguno de estos estados.\\
\\
Supongamos que se realiza la medición de una magnitud física del sistema representada por el operador $A$. El valor de expectación de $A$, suponiendo que cada $\left|\psi_i\right\rangle$ esté normalizado a la unidad, viene dado por

\begin{equation}\label{valorexp}
<A>=\sum_{n}p_n\left\langle \psi_n\left|A\right|\psi_n\right\rangle\,.
\end{equation}
\\
Es común describir la mezcla estadística de los vectores $\left|\psi_i\right\rangle$, mediante el llamado \emph{operador densidad}\index{subject}{Operador densidad}

\begin{equation}\label{densidad}
\rho=\sum_{n}p_n\left|\psi_n\right\rangle\left\langle \psi_n\right|\,.
\end{equation}
\\
El valor de expectación de un observable $A$ dado por (\ref{valorexp}) se reescribe ahora en términos del operador densidad

\begin{equation}\label{expectacion}
<A>=\textrm{tr}(\rho A)\,.
\end{equation}
\\
Si se toma $A=Id$, se obtiene la condición

\begin{equation}\label{norm}
\textrm{tr}(\rho)=1\,,
\end{equation}
\\
que está asociada a que los números $p_i$ son \emph{pesos estadísticos} y por lo tanto debe resultar

\begin{equation}\label{pesos}
\sum_{n}p_n=1\,,
\end{equation}
\\
ya que el sistema debe encontrarse en alguno de los estados $\left|\psi_i\right\rangle$.\\
\\
Como se ha dicho, el operador densidad $\rho$ es hermítico, tiene autovalores positivos y traza igual a la unidad. Estas propiedades, permiten probar que el espectro de $\rho$ es discreto y sus autovalores están comprendidos entre 0 y 1.\\
\\
Puesto que es suficiente dar $\rho$ para calcular todas las cantidades físicamente medibles y valores de expectación, se dice que dos mezclas estadísticas son idénticas si están representadas por el mismo operador densidad.

\subsubsection{Estados puros}\index{subject}{Estados puros}

El formalismo del operador densidad permite estudiar los casos puros como casos particulares de mezcla estadística. Si se sabe que el sistema se encuentra en un estado $\left|\alpha\right\rangle$, se puede escribir el operador densidad como

\begin{equation}\label{puro}
\rho=\left|\alpha\right\rangle\left\langle \alpha\right|\,,
\end{equation}
\\
que no es más que un proyector sobre el estado $\left|\alpha\right\rangle$, y por lo tanto debe resultar

\begin{equation}\label{rhocuadrado}
\rho^2=\rho\,.
\end{equation}
\\
En general, todo operador hermítico definido positivo de traza 1, posee la propiedad $\textrm{tr}\rho^2\leq1$. De las ecuaciones (\ref{rhocuadrado}) y (\ref{norm}) se ve trivialmente que si el estado del sistema es puro, entonces debe ser

\begin{equation}\label{rhocuadrado1}
\textrm{tr}(\rho^2)=1\,.
\end{equation}
\\
Se prueba sencillamente que $\rho$ representa un caso puro sí y sólo sí vale la ecuación (\ref{rhocuadrado1}).\\
\\
En conclusión, siempre es posible representar el estado de un sistema mediante su operador densidad, conociéndose el estado completa o incompletamente. Dado este operador es posible determinar todas las cantidades físicamente medibles utilizando la ecuación (\ref{expectacion}).

\subsubsection{Operador densidad reducido}\label{red}\index{subject}{Operador densidad reducido}

El concepto de \emph{operador densidad reducido} fue introducido por P. Dirac en 1930. Considérense dos sistemas $A$ y $B$ con espacios de Hilbert $H_A$ y $H_B$ respectivamente y supóngase que el estado del sistema completo es $\left|\psi\right\rangle\in H_A\otimes H_B$. Se introduce una base $\left|i,j\right\rangle=\left|i\right\rangle\otimes\left|j\right\rangle$ del espacio $H_A\otimes H_B$, con lo que $\left|\psi\right\rangle$ se escribe como $\sum\left|\psi\right\rangle=\lambda_{kl}\left|k,l\right\rangle$, siendo $\sum\left|\lambda_{kl}\right|^2=1$. En general, no se puede decir que el subsistema $A$ se encuentra en un estado puro. Sin embargo, puede definirse el operador densidad reducido al subsistema $A$ como

\begin{equation}\label{reducido}\index{subject}{Operador densidad reducido}
\rho_A=\textrm{tr}_B\left|\psi\right\rangle \left\langle \psi\right|=\sum_l\lambda_{kl}\lambda_{il}^*\left|k\right\rangle \left\langle i\right|\,,
\end{equation}
\\
y los valores de expectación de operadores $O:H_A\rightarrow H_A$ vendrán dados por

\begin{equation}\label{expectacionred}
<O>=\textrm{tr}(\rho_A O)\,.
\end{equation}
\\
Es interesante notar que cualquier operador densidad puede expresarse como estado reducido de un operador densidad puro. En efecto, consideremos un sistema caracterizado por el operador densidad $\rho$ y supongamos que los autovalores del mismo son $\lambda_i$, con lo que podemos escribir

\begin{equation}\label{ejreduccion}
\rho= \lambda_i\left|i\right\rangle\left\langle i\right|\,,
\end{equation}
\\
perteneciendo los estados $\left|i\right\rangle$ al espacio de Hilbert $H$ del sistema. Considérese una base $\left|i,j\right\rangle=\left|i\right\rangle\otimes\left|j\right\rangle\in H_A \times H_B$ ($H_A=H_B=H$). Se define

\begin{equation}\label{producto}
\rho_1=\sum \sqrt{\lambda_{i}\lambda_{j}}\left|i,i\right\rangle\left\langle j,j\right|=\left(\sum\sqrt{\lambda_i}\left|i,i\right\rangle\right)\left(\sum\sqrt{\lambda_j}\left\langle j,j\right|\right)\,,
\end{equation}
\\
Es sencillo ver que $\textrm{tr}({\rho_1}^2)=1$, por lo que el estado que representa $\rho_1$ es puro (describe al estado $\sum\sqrt{\lambda_i}\left|i,i\right\rangle$). Además, resulta

\begin{equation}\label{reduccion}
\rho= \textrm{tr}_B\rho_1\,.
\end{equation}
\\
donde $\textrm{tr}_B$ indica que hay trazar sobre el espacio de Hilbert $H_B$, como se ha definido en (\ref{reducido}).\\
\\
Una propiedad interesante surge de considerar un sistema compuesto por dos subsistemas A y B. Si el estado total del sistema $\rho_{AB}$ es puro, entonces, los autovalores no nulos de los operadores densidad reducidos $\rho_A$ y $\rho_B$ son los mismos. Esto puede demostrarse viendo que vale la igualdad $\textrm{tr}(\rho_A^n)=\textrm{tr}(\rho_B^n)$ para toda potencia $n$ y consecuentemente, los autovalores no nulos de $\rho_1$ y $\rho_2$ y sus multiplicidades coinciden.

\subsection{Entropía de von Neumann}\label{neumann1}\index{subject}{Entropía de von Neumann}

La forma más natural de definir la entropía de un sistema cuántico que se encuentra en un estado representado por el operador densidad $\rho$ es

\begin{equation}\label{neumann}\index{subject}{Entropía de von Neumann}
S(\rho)=-k_B \textrm{tr}(\rho \ln \rho)\,,
\end{equation}
\\
o sea, $S=-k_B \sum_{i}\lambda_i \ln \lambda_i$, donde $\lambda_i$ son los autovalores de $\rho$. Esta fórmula es debida a J. von Neumann (1927) y generaliza la expresión (\ref{ent-est}) de la entropía del caso clásico al cuántico. Se comentó que la definición (\ref{ent-est}) establecía una relación entre la variable de estado $S$ y la ''cantidad de desorden'' del sistema. Este grado de desorden está asociado a la cantidad de microestados posibles que pueden generar un estado con las mismas propiedades macroscópicas. En mecánica cuántica, el ''número de microestados'' puede interpretarse como el número de estados puros en los que se puede encontrar al sistema. Para ver esto, considérese por ejemplo un sistema cuántico que puede hallarse con la misma probabilidad en un número $\Omega$ de estados puros. El operador densidad del sistema es $\rho=(1/\Omega)P$, donde $P$ es un operador que proyecta vectores sobre un subespacio de dimensión $\Omega$. La entropía resulta $S=-k_B \textrm{tr}(\rho \ln \rho)=k_B \ln(\Omega)$ y se observa la similitud entre las ecuaciones (\ref{ent-est}) y (\ref{neumann}).\\
\\
La entropía de von Neumann es la única cantidad para la cual aparece esta semejanza con (\ref{ent-est}) y para la cual se cumplen ciertas propiedades\footnote{Tales como la aditividad y subaditividad, y diversas propiedades de mezclado.} que se desea que ''herede'' una entropía definida en un contexto cuántico, de las propiedades conocidas para el caso clásico.\\
\\
De la propia definición de la entropía de von Neumann, se sigue que la misma sólo es nula cuando el operador densidad que describe el estado tiene sólo un autovalor no nulo e igual a la unidad, es decir, cuando el estado es puro.\\
\\
De ahora en adelante se considera $k_B=1$.

%\subsection{Entropía y teoría de la información}

\section{Entrelazamiento cuántico}\index{subject}{Entrelazamiento cuántico}

El \textit{entrelazamiento} es un fenómeno cuántico, sin equivalente clásico, en el cual los estados de dos o más subsistemas se deben describir haciendo referencia a los estados del sistema total, incluso cuando la separación entre los subsistemas es grande.\\
\\
Las mediciones realizadas sobre algún observable de un sistema que está entrelazado con otros parecen influenciar instantáneamente a estos. Por ejemplo, si tenemos un sistema de dos fotones con espín total nulo y los separamos infinitamente, la medición del espín de uno de ellos determinará de forma unívoca el espín del otro. Esto parecería sugerir que alguna influencia debería estar propagándose "instantáneamente" entre los sistemas, a pesar de la separación entre ellos, lo que violaría la velocidad máxima de propagación de las interacciones.\\
\\
El entrelazamiento cuántico fue en un principio utilizado por A. Einstein, B. Podolsky y N. Rosen (EPR)\,\cite{einstein} como un argumento para intentar probar la incompletitud de la mecánica cuántica como teoría física, alegando que las correlaciones predichas por la mecánica cuántica son inconsistentes con el Principio del Realismo Local \footnote{El Principio de Realismo Local es una conjunción entre el Principio de Localidad y la asunción de que todas las magnitudes físicas tienen valores preexistentes para cada medición incluso antes de que se realice la medición. En el contexto planteado en \cite{einstein}, se refiere a que cada partícula debe tener un estado bien definido, sin que sea necesario hacer referencia a otros sistemas distantes.}.\\
\\
En 1964, un trabajo presentado por J. Bell \cite{bell} permitió cuantificar matemáticamente en forma de desigualdades las implicaciones teóricas planteadas en el trabajo de EPR. El hecho de que las desigualdades de Bell sean violadas\footnote{Hecho que se ha comprobado experimentalmente, en primera oportunidad por A. Aspect en 1982 \cite{aspect}.} provee evidencia empírica a favor de la mecánica cuántica y en contra del Realismo Local.

\subsection{La Paradoja EPR}

En el trabajo original de Einstein, Podolsky y Rosen se hace un análisis del entrelazamiento que presenta un sistema de dos partículas, que interactuaron durante un intervalo de tiempo determinado y luego son separadas espacialmente, en términos del momento lineal y la posiciones de las partículas. Una situación en la que se puede visualizar el fenómeno de entrelazamiento en forma más sencilla fue introducida por D. Bohm en 1951, y consiste en pensar en un sistema formado por dos partículas de espín 1/2 en un estado inicial de espín total igual a cero. Supongamos que el estado de espín total inicial del sistema se puede escribir como

\begin{equation}\label{espinini}
\left|\chi\right\rangle=\frac{1}{\sqrt{2}}\left(\left|\uparrow\downarrow\right\rangle-\left|\downarrow\uparrow\right\rangle\right)\,,
\end{equation}
\\
donde $\left|\uparrow\downarrow\right\rangle=\left|\uparrow\right\rangle\otimes\left|\downarrow\right\rangle$ (este podría ser, por ejemplo, el caso de un par de electrones con un estado orbital simétrico). Una de las partículas se aleja lo suficiente de la otra como para asegurar que la interacción entre ambas sea nula. Si un observador mide el espín de una de estas partículas y la encuentra, por ejemplo, en el estado de espín positivo, este observador sabe inmediatamente que la partícula que está alejada de él tiene que encontrarse en el estado de espín negativo. Esto está asociado al colapso de la función de onda total de las dos partículas después de la medición; si la partícula $1$ tiene un espín positivo, entonces el estado inicial colapsa a

\begin{equation}\label{espinfin}
\left|\chi\right\rangle=\left|\uparrow\downarrow\right\rangle\,,
\end{equation}\
\\
lo que indica que el espín de la partícula $2$ tiene que ser negativo. A pesar de haber medido una propiedad de la partícula $1$, la partícula $2$ es ''afectada'' por la medición. En realidad, esto dice que los sistemas de muchas partículas que estuvieron interactuando durante un tiempo no pueden ser descriptos luego como sistemas desconectados o independientes, aún a tiempos posteriores de que la interacción se suprima. Esto es lo que constituye el fenómeno del entrelazamiento cuántico.


\subsection{Medidas de entrelazamiento}

Hasta ahora se ha introducido una idea de lo que representa el fenómeno de entrelazamiento. Sin embargo, no se ha dado aún un criterio claro que permita decir si un sistema se encuentra o no entrelazado. Supóngase que se tiene un sistema constituído por dos subsistemas $A$ y $B$. Se dice que el estado del sistema total es \textbf{separable} si su operador densidad se puede escribir como

\begin{equation}\label{separable}
\rho_{AB}=\underset{\lambda}\sum p_{\lambda}\rho^{\lambda}_A\otimes\rho^{\lambda}_B\,,
\end{equation}
\\
donde los números $p_i$ son pesos estadísticos; un estado separable describe sólo correlaciones clásicas entre $A$ y $B$. Así, un sistema entrelazado es un sistema en un estado no separable, es decir, que no puede escribirse como (\ref{separable}). Varias medidas de entrelazamiento cuántico entre dos sistemas $A$ y $B$ han sido propuestas y se denotan $E(A,B)$. En general, $E(A,B)$ es una cantidad que es muy difícil de calcular, ya que su definición involucra determinar ínfimos o supremos sobre conjuntos infinitos, que no son sencillos de evaluar. Por este motivo, suele ser útil trabajar con otras cantidades (medidas de entrelazamiento) que guardan alguna relación conocida con $E(A,B)$. Un ejemplo de estas cantidades es la \textbf{información mutua} $I(A,B)$ que es presentada en la sección \ref{secmutua}. La información mutua es una medida de entrelazamiento muy importante dado que establece una cota máxima a $E(A,B)$; además, si el estado $\rho_{AB}$ es puro, para todas las medidas de entrelazamiento resulta $E(A,B)=\frac{1}{2}I(A,B)$. Existen muchas otras medidas de entrelazamiento  tales como el entrelazamiento de formación, de destilado, condicional y el \textit{squashed entanglement}. En este trabajo sólo se considera la información mutua por diversas propiedades que se destacan con detalle en la sección \ref{secmutua}.

\subsection{Entropía de entrelazamiento}

Ya se comentó que el entrelazamiento se refiere a las correlaciones existentes entre dos sistemas aún luego de que los mismos no están interactuando, y también se discutió sobre algunas medidas de entrelazamiento. Una cantidad que da cuenta del grado de entrelazamiento entre dos sistemas es la llamada \textbf{entropía de entrelazamiento}.\\
\\
Supóngase que se tiene un sistema compuesto de dos subsistemas A y B, en un estado total puro. Todas las mediciones que se realizan sobre el subsistema A (B) se pueden describir en términos del operador densidad reducido $\rho_A$ ($\rho_B$). Se define la entropía de entrelazamiento $S_A$ entre el subsistema A y el B como la entropía de von Neumann (\ref{neumann}) para la matriz densidad $\rho_A$

\begin{equation}\label{entrelazamiento}
S_A=S(\rho_A)\,.
\end{equation}
\\
Es sencillo ver que la entropía de entrelazamiento $S_A$ coincide con la entropía de entrelazamiento $S_B$, definida a partir de la matriz densidad reducida $\rho_B$, si el estado total del sistema compuesto es puro\footnote{Esta igualdad sale como una consecuencia directa de la igualdad de los autovalores de $\rho_A$ y $\rho_B$ que se probó en la sección~\ref{red}.}. La igualdad entre $S_A$ y $S_B$ sólo es cierta cuando el estado del sistema compuesto es puro, en cuyo caso la entropía $S_{A\cup B}$ es nula. Esto pone de manifiesto el hecho de que, en general, la entropía no es aditiva. En este caso puro se tiene $S(A)=E(A,B)=\frac{1}{2}I(A,B)$ para toda $E$.\\
\\
Una motivación para decir que $S(A)$ es una medida del entrelazamiento entre $A$ y $B$ es la siguiente. En la sección~\ref{neumann1} se comentó que la entropía de von Neumann era nula sólo si el estado representado por el operador densidad era puro. Si el estado total del sistema A+B es puro, y además el estado representado por $\rho_A$ es puro, entonces, por la igualdad entre $S_A$ y $S_B$, el estado representado por $\rho_B$ también debe ser puro. En este caso, el estado total es un estado producto

\begin{equation}
\left|\Psi_{A+B}\right\rangle=\left|\Psi_A\right\rangle\otimes\left|\Psi_B\right\rangle\,,
\end{equation}
\\
que es separable, y el fenómeno de entrelazamiento no se manifiesta, dado que no hay correlaciones entre el sistema A y el B. Este hecho, hace plausible la definición (\ref{entrelazamiento}) de la entropía de entrelazamiento como la entropía de von Neumann asociada al operador densidad reducido $\rho_{A}$, ya que cuando no hay correlaciones entre los dos subsistemas (es decir, cuando los sistemas no están entrelazados) $S_A$ se anula.

\subsubsection{Cálculo de entropía de entrelazamiento}\label{discreto}

En la literatura se exploran básicamente dos acercamientos para calcular la entropía de entrelazamiento en teorías cuánticas de campos libres: el formalismo de tiempo Euclídeo y el de tiempo real. En este trabajo utilizaremos el formalismo de tiempo real, que apunta a calcular directamente el operador densidad reducido correspondiente al estado global de vacío en término de correladores de los campos. Para ello, se comienza con una versión discreta de la teoría de campos y luego se toma el límite al continuo. Los primeros cálculos de entropía de entrelazamiento utilizando el formalismo de tiempo real fueron realizados en \cite{bombelli}, varios años antes de que se desarrolase el formalismo Euclídeo, y si bien aún no ha sido tan explorado como este último, se cree que es más adecuado para realizar generalizaciones \cite{huerta}. Por ejemplo, puede ser utilizado para realizar cálculos que involucren conjuntos espaciales no contenidos en un único hiperplano espacial en espacio de Minkowski, para lo cual el formalismo Euclídeo no podría aplicarse.\\
\\
A continuación, se pretende calcular la entropía de entrelazamiento para el estado fundamental de un sistema reducido a una región $V$ utilizando el formalismo de tiempo real. Se recuerda que el operador densidad reducido a una región $V$ del espacio, representa al estado que reproduce los valores de expectación en el vacío de operadores $O_V$ localizados en $V$, es decir

\begin{equation}\label{valores}
\left\langle O_V\right\rangle =\textrm{tr}(\rho_V O_V)\,.
\end{equation}\\

\begin{itemize}

\item \textbf{Bosones}

Los operadores hermíticos coordenada $\phi_i$ y su momento conjugado $\pi_j$ satisfacen las siguientes relaciones de conmutación

\begin{equation}
[\phi_i,\pi_j]=i\delta_{ij}\, ,\,\,\,[\phi_i,\phi_j]=[\pi_i,\pi_j]=0\,.
\end{equation}
\\
Supóngase que se conocen las funciones de correlación de dos puntos dentro de $V$

\begin{equation}\label{corres1}
\left\langle \phi _{i}\phi _{j}\right\rangle =X_{ij}\, ,\,\,\,\left\langle \pi _{i}\pi _{j}\right\rangle =P_{ij}\,,
\end{equation}
\\
\begin{equation}\label{corres2}
\left\langle \phi _{i}\pi _{j}\right\rangle =\left\langle \pi _{j}\phi _{i}\right\rangle^{*}= \frac{i}{2}\delta_{ij}\,.
\end{equation}
\\
La última ecuación podría parecer un poco arbitraria y en realidad puede generalizarse. Sin embargo, a los efectos de trabajar con el estado de vacío es suficiente pedir que valga (\ref{corres2}). De las ecuaciones en (\ref{corres1}) se deduce que las matrices $X$ y $P$ son hermíticas y tienen autovalores positivos. Además, es sencillo demostrar que el producto

\begin{equation}\label{mayor}
X\cdot P\geq \frac{1}{4}\,,
\end{equation}
\\
donde debe entenderse que la condición es para los autovalores de las matrices $X$ y $P$. Los correladores de más de dos puntos pueden obtenerse a partir de estos, en virtud del teorema de Wick

\begin{equation}\label{wickboson}
\left\langle Of_{i_{1}}f_{i_{2}}...f_{i_{2k}}\right\rangle =\frac{1}{2^{k}k!
}\underset{\sigma }{\sum }\left\langle Of_{i_{\sigma (1)}}f_{i_{\sigma
(2)}}\right\rangle ...\left\langle Of_{i_{\sigma (2k-1)}}f_{i_{\sigma
(2k)}}\right\rangle \,,
\end{equation}
\\
donde la suma es sobre todas las permutaciones $\sigma$ de índices, $f_i$ puede ser $\phi_i$ o $\pi_i$ y $O$ es un operador de orden específico, por ejemplo, podría indicar ordenar los productos dentro de los valores de expectación con las coordenadas a la izquierda y los momentos a la derecha.\\
\\

Se consideran operadores de creación y destrucción $a_l$, $a_l^{\dagger}$, con $[a_i$, $a_j^{\dagger}]=\delta_{ij}$, que se expresan como combinaciones lineales de los $\phi_i$ y $\pi_j$

\begin{equation}\label{creadest1}
\phi_i=\alpha_{ij}^*a_j^{\dagger}+\alpha_{ij}a_j\,,
\end{equation}
\\
\begin{equation}\label{creadest2}
\pi_i=-i\beta_{ij}^*a_j^{\dagger}+i\beta_{ij}a_j\,.
\end{equation}
\\

Las relaciones de conmutación entre las coordenadas y los momentos dan

\begin{equation}
\alpha^*\beta^T+\alpha\beta^{\dagger}=-1\,.
\end{equation}
\\

Se propone la siguiente forma para el operador densidad reducido

\begin{equation}\label{matrizdens}
\rho_V=K\,e^{\cal{H}}=K\,e^{-\sum \epsilon_l a_l^{\dagger} a_l}\,,
\end{equation}
\\

siendo $K=\prod\left(1-e^{-\epsilon_l}\right)$ una constante de normalización. Con esta forma del operador densidad, se satisface la propiedad (\ref{wickboson}). Utilizando la ecuación (\ref{valores}) y la forma explícita del operador densidad reducido, se puede hallar, a partir de las relaciones (\ref{corres1}) y (\ref{corres2})

\begin{equation}
\alpha^*n\beta^T-\alpha(n+1)\beta^{\dagger}=\frac{1}{2}\,,
\end{equation}
\\
\begin{equation}
\alpha^*n\alpha^T+\alpha(n+1)\alpha^{\dagger}=X\,,
\end{equation}
\\
\begin{equation}
\beta^*n\beta^T-\beta(n+1)\beta^{\dagger}=P\,,
\end{equation}
\\

siendo $n$ la matriz diagonal dada por

\begin{equation}
n_{k}=\left\langle a_k^{\dagger}a_k\right\rangle=(e^{\epsilon_k}-1)^{-1}\,.
\end{equation}
\\

De estas ecuaciones, se obtiene que $\alpha=\alpha_1 U$y $\beta=\beta_1 U$, siendo $U$ unitaria y diagonal, y $\alpha_1$ y $\beta_1$ reales. La matriz $U$ puede reabsorberse en la definición de los $a_i$, por lo que ponemos $U=1$. Así $\alpha=-\frac{1}{2}(\beta^T)^{-1}$ y

\begin{equation}\label{loqueda}
\alpha\frac{1}{4}(2n+1)^2\alpha^{-1}=XP\,.
\end{equation}
\\

Al ser $\alpha\frac{1}{4}(2n+1)^2\alpha^{-1}$ semejante a $\frac{1}{4}(2n+1)^2$, de (\ref{loqueda}) se puede leer el espectro del operador densidad reducido en términos del espectro de $XP$

\begin{equation}
\frac{1}{2}\textrm{ctgh}(\epsilon_k /2)=\nu_k\,,
\end{equation}
\\

donde $\nu_k$ son los autovalores de

\begin{equation}
C=\sqrt{XP}\,.
\end{equation}
\\
Invirtiendo las relaciones (\ref{creadest1}) y (\ref{creadest2}) y reemplazando en (\ref{matrizdens}), el operador densidad reducido queda

\begin{equation}
\rho_V=K\,e^{-\sum(M_{ij}\phi_i\phi_j+N_{ij}\pi_i\pi_j})\,,
\end{equation}
\\

donde

\begin{equation}
M=\frac{1}{4}\alpha^{-1\,T}\epsilon \alpha^{-1}=\frac{P}{2C}\ln\left( \frac{C+1/2}{C-1/2}\right)\,,
\end{equation}

\begin{equation}
N=\alpha\epsilon\alpha^T=\frac{1}{2C}\ln\left( \frac{C+1/2}{C-1/2}\right)X\,,
\end{equation}
\\

siendo $\epsilon$ la matriz diagonal de los $\epsilon_k$. La entropía, dada por (\ref{neumann}), queda

\begin{equation}
S=\textrm{tr}\left[ \left( C+1/2\right) \ln \left( C+1/2\right) -\left( C-1/2\right)
\ln \left( C-1/2\right) \right]\,,
\end{equation}

que resulta positiva en virtud de la ecuación (\ref{mayor}).\\
\\
Para el estado fundamental de un hamiltoniano de la forma $H=\frac{1}{2}\sum \pi_i^2+\frac{1}{2}\sum \phi_iK_{ij}\phi_j$, los correladores (\ref{corres1}) están dados por

\begin{equation}
X_{ij}=\frac{1}{2}(K^{-1/2})_{ij}\,,
\end{equation}

\begin{equation}
P_{ij}=\frac{1}{2}(K^{1/2})_{ij}\,.
\end{equation}
\\
Para el estado global, se tiene $X\cdot P=1/4$, que tiene entropía nula, como corresponde para un estado puro.\\
\\
Esta formulación pone en evidencia el hecho de que para hallar la matriz densidad reducida sólo es necesario conocer los correladores dentro de $V$. La extensión al continuo del caso bosónico no ha sido muy explorada aún, dado que el problema involucra núcleos más singulares que los que aparecen en el caso fermiónico.\\

\item \textbf{Fermiones}

Los operadores $\psi_i^{\dagger}$ y $\psi_j$ satisfacen las relaciones de anticonmutación

\begin{equation}
\left\{ \psi _{i},\psi _{j}^{\dagger}\right\} =\delta _{ij}\,.
\end{equation}
\\
Supóngase que los correladores de dos puntos son

\begin{equation}\label{fermion1}
\left\langle \psi_{i}\psi_{j}^{\dagger}\right\rangle =C_{ij}\, ,\,\,\,\left\langle \psi_{i}^{\dagger}\psi_{j}\right\rangle =\delta_{ij}-C_{ij}\,,
\end{equation}
\\\begin{equation}\label{fermion2}
\left\langle \psi_{i}\psi_{j}\right\rangle =\left\langle \psi_{i}^{\dagger}\psi_{j}^{\dagger}\right\rangle=0\,.
\end{equation}
\\

Se asume aquí también que el teorema de Wick es válido y todos los correladores de más de dos puntos que no se anulan se pueden obtener a partir de los correladores de dos puntos como

\begin{equation}
\left\langle \psi _{i_{1}}...\psi _{i_{k}}\psi _{j_{1}}^{\dagger}...\psi
_{j_{k}}^{\dagger}\right\rangle =(-1)^{k(k-1)/2}\underset{\sigma }{\sum }
\epsilon _{\sigma }\underset{q=1}{\overset{k}{\prod }}\left\langle \psi
_{i_{q}}\psi _{j_{\sigma (q)}}^{\dagger}\right\rangle\,,
\end{equation}
\\

donde la suma se realiza sobre todas las permutaciones de los índices $j_1$, $j_2$, ..., $j_k$, y $\epsilon_\sigma$ es el signo de la permutación. De las ecuaciones (\ref{fermion1}) se ve que los autovalores de $C$ se encuentran en el intervalo $[0,1]$. Si $V$ es el espacio total, $C$ es un proyector y sus autovalores son $0$ y $1$.\\
\\
Al igual que en el caso bosónico, los correladores dentro de $V$ calculados haciendo uso del operador densidad reducido satisfacen la propiedad de Wick si se tiene

\begin{equation}\label{latercera}
\rho_V=K\,e^{-\cal{H}}=K\,e^{-\sum H_{ij}\psi_i^{\dagger}\psi_j}\,.
\end{equation}
\\

Como $\rho_V$ es hermítico, $H$ también debe ser hermítico. El exponente de la ecuación anterior se puede diagonalizar entonces utilizando la transformación de Bogoliuvov $d_l=U_{lm}\psi_m$, siendo $U$ unitaria (para que resulte ${d_i,d_j^{\dagger}}=\delta_{i,j}$. $U$ se elije de modo que $UHU^{\dagger}=\epsilon$, siendo $\epsilon$ una matriz diagonal de los autovalores de $H$. Se tiene

\begin{equation}\label{lacuarta}
\rho_V=\prod\frac{e^{-\epsilon_l d_l^{\dagger}d_l}}{(1+e^{-\epsilon_l})}\,;
\end{equation}
\\
nótese que de la ecuación anterior se obtiene el valor de la constante $K=\textrm{det}=(1+e^{-H})^{-1}$. La relación entre los autovalores de $C$ y los de $H$ sale de las ecuaciones (\ref{valores}), (\ref{fermion1}), (\ref{latercera}) y (\ref{lacuarta}). Si se nota con $\nu_l$ a los autovalores de $C$ se obtiene la siguiente relación

\begin{equation}
e^{\epsilon_l}=\frac{\nu_l}{1-\nu_l}\,,
\end{equation}
\\
que se puede poner en notación matricial como

\begin{equation}
H=-\ln(C^{-1}-1)\,.
\end{equation}
\\
El cálculo de la entropía de von Neumann para este operador densidad reducido puede evaluarse como una suma sobre cada modo independiente de $H$ autovalor $\epsilon_l$, obteniéndose

\begin{equation}
S=-\textrm{tr}\left[ \left( 1-C\right) \ln \left( 1-C\right) +C\ln \left( C\right)\right]\,.
\end{equation}
\end{itemize}

\section{Entropía en teorías relativistas}

\subsection{Problemas de la entropía en teorías de campos}

El estado relevante para el cálculo de valores de expectación de observables en una región $V$ es el operador densidad reducido $\rho_V$. A partir del operador densidad reducido es posible evaluar la entropía geométrica en la región, definida a partir de la ecuación (\ref{neumann}) para el estado de vacío. Cuando uno considera teorías relativistas, la entropía geométrica resulta ser divergente \cite{bombelli,hooft}. Estas divergencias aparecen como consecuencia del entrelazamiento presente en las fluctuaciones del vacío alrededor de la frontera de $V$ (ver figura \ref{fluctuaciones}). El proceso de localización conlleva inevitablemente la creación de pares de partícula-antipartícula. Si una de las partículas se encuentra dentro de $V$ y la otra fuera, para hallar el operador densidad reducido $\rho_V$, la partícula dentro de $V$ queda como una partícula real mientras los grados de libertad asociados a la otra se trazan. Dada la naturaleza ultravioleta del problema, los términos divergentes aparecen en el cálculo de la entropía de entrelazamiento también para los estados excitados de energía finita reducidos a la región $V$.\\
\\
\begin{figure}[h]
\begin{center}
\includegraphics[width=5cm]{fluctuaciones.jpg}
\end{center}
\caption{\textbf{Fluctuaciones del vacío}. El proceso de localización en teorías relativistas lleva a la creación de pares de partícula-antipartícula. El entrelazamiento en estos pares es la causa de las contribuciones divergentes a la entropía geométrica.} \label{fluctuaciones}
\end{figure}

En el capítulo \ref{ch:plano} de este trabajo se calcula explícitamente la entropía geométrica para una teoría de campos y se encuentran estas divergencias. A modo de ejemplo sin embargo, y para visualizar el rol de los términos divergentes y finitos en la entropía, se muestra la entropía de un fermión de masa nula en $1+1$ dimensiones a temperatura $T$. El cálculo fue realizado en \cite{cardy}, en un intervalo espacial de longitud $L$, utilizando el formalismo de tiempo euclídeo. El resultado hallado en \cite{cardy} para la entropía es

\begin{equation}\label{tfinita}
S=\frac{1}{3}\ln\left[\frac{1}{\pi \epsilon T}\textrm{sinh}\left(\pi L T\right)\right]\,,
\end{equation}
\\
donde $\epsilon$ es un \textit{cutoff} ultravioleta con unidades de distancia. En el límite en que $L T\rightarrow \infty$, la ecuación (\ref{tfinita}) da

\begin{equation}\label{finnn}
S\approx\frac{1}{3}\ln(\epsilon)+\ln\left(\frac{1}{T}\right)+\frac{\pi}{3}L T\,,
\end{equation}
\\
donde el último sumando de (\ref{finnn}) dice que la entropía crece en forma proporcional al volumen, como suele ocurrir para un estado térmico. Para $L T\rightarrow 0$ se obtiene

\begin{equation}
S\approx-\frac{1}{3}\ln\left(\frac{L}{\epsilon}\right)\,,
\end{equation}
\\
que es un resultado que también puede obtenerse independientemente utilizando el formalismo de tiempo real, para la misma teoría con temperatura nula (este cálculo, utilizando el formalismo de tiempo real, se realiza en el capítulo 4). El término $\frac{\pi}{3}L T$ se obtendría también si uno pusiera al sistema en una caja con condiciones de borde a temperatura $T$, tomando el límite de $L$ grande. De (\ref{finnn}), se ve que en este límite, es posible separar el término proporcional al volumen de la parte divergente. Se dice entonces que este término es universal, o sea, independiente del \textit{cutoff} o las condiciones de borde que se impongan en la caja.

\subsection{Ambigüedades de la entropía en la radiación de Hawking}

En $d$ dimensiones espaciales, para cualquier teoría de campos se debería tener

\begin{equation}\label{ultimaec}
S(V)=g_{d-1}[\partial V]\epsilon^{-(d-1)}+...+g_1 [\partial V]\epsilon^{-1}+g_0[\partial V]\ln(\epsilon)+S_0(V)\,,
\end{equation}
\\
siendo $S_0(V)$ una contribución finita, $\epsilon$ un \textit{cutoff} ultravioleta y las $g_i$ funciones locales extensivas del borde $\partial V$~\footnote{Esto está asociado a que los modos de corta longitud de onda que se encuentran entrelazados entre la región exterior y la interior a $V$ sólo pueden aportar en el borde y de manera local, es decir como una integral sobre el borde.}. El coeficiente del primer término $g_{d-1}[\partial V]$ es entonces, en el caso sin masa, proporcional a la $d-1$ potencia del tamaño de $V$ y suele asociarse a una ley del área para la entropía de entrelazamiento. Los términos proporcionales a $g_i$ para $i>0$ no tienen una interpretación física en teoría de campos, dado que no están asociados a cantidades independientes de la regularización. Sin embargo, sí se espera que el coeficiente $g_0$ del término logarítmico sea universal, es decir, independiente de la regularización.\\
\\
En general, estos términos divergentes son ambiguos. Sin embargo, por ejemplo para el caso de un estado térmico, la diferente dependencia de la entropía térmica con el volumen $S_T\sim V T$ permitiría extraer este término universal de la entropía. Un situación muy diferente se da en casos en los cuales la entropía se encuentra muy diluída, como ocurre con la entropía de la radiación de Hawking en los agujeros negros. Estos son objetos relativamente fríos, que emiten radiación a una temperatura $T\sim r_S^{-1}$ (siendo $r_s$ el tamaño del agujero negro; en el capítulo \ref{ch:agujeros}, se dan más detalles acerca de los agujeros negros). La entropía emitida en este caso viene dada heurísticamente como

\begin{equation}
S\approx T^3\cdot V=T^3\times\textrm{área\,de\,emisión}\times\textrm{tiempo}=\frac{R_{shell}}{r_s}\,,
\end{equation}
\\
que no puede separarse de los términos divergentes $S\sim\frac{R_{shell}^2}{\epsilon^2}+\frac{R_{shell}}{\epsilon}+...$. Este problema puede subsanarse utilizando alguna otra medida de información, como se verá en la siguiente sección.

\subsection{Medidas de información en teorías de campos. Información mutua}\label{secmutua}

Se ha comentado que la localización estricta de un estado en una región del espacio, en teorías relativitas, da lugar a la formación de pares partícula-antipartícula y que en la aparición de estos modos de alta energía se encuentra el origen de las divergencias en la entropía de entrelazamiento. Una contribución divergente similar aparecerá en cualquier cálculo de la entropía en una región separada de otra por un horizonte causal, como es el caso de los agujeros negros. Sin embargo, la noción de entrelazamiento entre dos regiones distintas puede definirse de modo preciso en teoría de campos, aún en presencia de gravitación. Las medidas de entrelazamiento entre regiones disjuntas no presentan divergencias y son, en principio, calculables en la teoría semiclásica.\\
\\
Es posible realizar una substracción en la entropía de entrelazamiento del vacío para eliminar las divergencias provenientes de las fluctuaciones del vacío. Sin embargo, no se puede simplemente llevar a cero el valor de esta entropía, dado que existen cantidades finitas universales (independientes de la regularización) que se pueden obtener a partir de ella. Una de esas cantidades es la \textbf{información mutua}

{\small
\begin{equation}\label{infomutua}
I(A,B)=S(A)+S(B)-S(A\cup B)\,,
\end{equation}}
\\

entre dos conjuntos disjuntos (ver figura \ref{mutua}) $A$ y $B$. Nótese que los términos divergentes, que están asociados a los bordes de las regiones se sustraen en (\ref{infomutua}). En estadística, la información mutua da una medida a la información compartida por dos sistemas. La información mutua es una cantidad bien definida en teoría de campos, con el único requerimiento de que exista una separación no nula entre las regiones $A$ y $B$, y mide el grado de no extensividad que tiene la entropía $S$.\\
\\
\begin{figure}[h]
\begin{center}
\includegraphics[width=5cm]{mutua.jpg}
\end{center}
\caption{\textbf{Información mutua}. Para dos regiones $A$ y $B$ disconexas, como las que se muestra en la figura, es posible definir una cantidad universal de la que puede inferirse la entropía de entrelazamiento.} \label{mutua}
\end{figure}

Si la región $B$, por ejemplo, se extendiera a todo el espacio de modo de tender a cubrir la región $-A$, y el contorno de $B$ se aproximara al de $A$ desde afuera, se obtendría $S(A)\approx S(-B)=S(B)$ y $S(A\cup B)\approx 0$ y, entonces

\begin{equation}\label{recupera}
I(A,B)\approx 2S(A)\,.
\end{equation}
\\
Así, la información mutua diverge del mismo modo que la entropía cuando los conjuntos se acercan uno al otro y, de algún modo, se reproducen las divergencias presentes en $S(A)$, pero ahora en forma independiente de la regularización.

\subsubsection{Propiedades de la información mutua}\label{sectripartita}

Para un sistema cuántico general, la función $I(A,B)$ es simétrica, adimensional y positiva. Si se considera un estado producto, dado por $\rho_{A\cup B}=\rho_A \otimes \rho_B$, la información mutua $I(A,B)$ se anula. Otra propiedad interesante es la de monotonía respecto al tamaño de los conjuntos

\begin{equation}\label{monoinfo}
I(A,B)\leq I(A,C)\,,\,\textrm{si}\,\,\,B\subseteq C\,.
\end{equation}
\\
Esta propiedad, indica que la información mutua varía suavemente con el conjunto y es una consecuencia de la propiedad de subaditividad fuerte de la entropía. También se tiene la siguiente desigualdad

\begin{equation}
I(A,B)\leq 2 \,\textrm{min}(S(A),S(B))\,.
\end{equation}
\\
También es posible definir la \textbf{información tripartita}

\begin{equation}\label{tripartita}
I(A|B,C)=I(A,B)+I(A,C)-I(A,B\cup C)\,,
\end{equation}
\\
que mide la información compartida entre $B$ y $C$ respecto de $A$. Por la propia definición de la información mutua (\ref{infomutua}), la información tripartita tiene simetría de permutación total

{\small
\begin{eqnarray}\label{triparentro}
&&I_3(A,B,C)\equiv I(A|B,C)=\\
&&S(A\cup B\cup C)-S(A\cup B)-S(B\cup C)-S(C\cup A)+S(A)+S(B)+S(C)\,.\nonumber
\end{eqnarray}}
\\
Así como la información mutua mide el grado de no extensividad de la entropía, la información tripartita, en virtud de la ecuación (\ref{tripartita}), mide el apartamiento de la extensividad de la información mutua. Nótese que a diferencia de $I(A,B)$, $I_3(A,B,C)$ puede ser tanto positiva o negativa, y es nula en particular cuando el estado total es puro. Sin embargo, la condición general que hace que la información mutua sea extensiva es aún desconocida.

%COSAS QUE PODRÍAN SERVIR Y QUE NO INCLUÍ
%
%Considérese un sistema compuesto por dos subsistemas A y B. El subsistema A (B) tendrá asociado para su descripción un Conjunto Completo de Observables que Conmutan (CCOC) cuyos autovalores identificaremos con $\alpha$ ($\beta$). Supóngase que el sistema total se encuentra en un estado puro dado por $\left|\alpha,\beta\right\rangle$. Consideremos ahora los subsistemas como entes separados. Todas las mediciones que se realizan sobre el subsistema A (B) se pueden describir en términos del operador densidad reducido $\rho_A$ ($\rho_B$), siendo

%\begin{equation}\label{sistA}
%\rho_A=\textrm{tr}_B\left|\alpha,\beta\right\rangle \left\langle\alpha,\beta\right|
%\end{equation}

%\begin{equation}\label{sistB}
%\rho_B=\textrm{tr}_A\left|\alpha,\beta\right\rangle \left\langle\alpha,\beta\right|
%\end{equation}\

%El hecho de que cada subsistema esté descripto por un operador y no por un estado puro no está relacionado con una falta de conocimiento del estado del sistema total. De hecho, en el caso que se está considerando, el estado total es puro y aún así los sistemas no estarán descriptos por estados puros en general. Ya se ha comentado que la entropía de Von Neumann definida en \ref{neumann} es nula sólo si el estado en consideración está descripto por un operador densidad asociado a un estado puro (que tiene sólo un autovalor no nulo). Por lo tanto, sólo cuando el estado total del sistema sea un estado producto

==> holo.tex <==
\chapter{\label{ch:holo}Entropía holográfica de entrelazamiento}

Muchas veces, los nuevos hallazgos de la física téorica aparecen al entender que dos conceptos diferentes se encuentran relacionados entre sí a un nivel más fundamental. Ejemplos de estas relaciones son las dualidades que vinculan dos aparentemente diferentes teorías cuánticas; en tales casos, los espacios de Hilbert y la dinámica de las dos teorías coinciden, a pesar de que los lagrangianos sean distintos. La dualidad Anti-de Sitter/Conformal Field Theory (AdS/CFT), es otro tipo de dualidad que relaciona una teoría de campos conforme en espacio plano con una teoría de cuerdas. Intuitivamente, la teoría de campos cuántica en espacio plano no aparenta ser una teoría cuántica de la gravedad. Sin embargo, la correspondencia AdS/CFT establece que las dos teorías son equivalentes.

En un contexto más general, la dualidad AdS/CFT es una realización precisa del principio holográfico. Este principio establece que en una teoría gravitatoria, el número de grados de libertad en cierto volumen $V$ escalea como el área de la superficie $\partial V$ del volumen dado. La teoría cuántica de la gravedad involucrada en la correspondencia está definida en general sobre una variedad de la forma AdS$\times X$, donde $X$ es un espacio compacto, y la teoría de campos conforme queda definida sobre el borde del espacio AdS.

En este capítulo introducimos a grandes rasgos las ideas generales que hay detrás de esta dualidad y, en particular, estudiamos una conjetura que permite calcular la entropía de entrelazamiento en la teoría de campos a partir de un cálculo geométrico en la teoría gravitatoria.

\section{Correspondencia AdS/CFT}

Como mencionamos en la introducción al capítulo, la correspondencia AdS/CFT relaciona teorías gravitatorias en espacios asintóticamente Anti-de Sitter con teorías de campos conformes. Una realización específica de esta dualidad se da para las teorías de Super Yang-Mills (SYM) con ${\cal N}=4$ en $3+1$ dimensiones y la teoría de supercuerdas tipo $IIB$ en AdS$_5 \times S^5$. La correspondencia AdS$_5$/CFT$_4$ (en su versión más fuerte) establece que la teoría de SYM ${\cal N}=4$, con grupo de simetría $SU\left(N\right)$ y constante de acoplamiento $g_{YM}$ es dinámicamente equivalente a teoría de supercuerdas tipo $IIB$, donde la longitud de las cuerdas es $l_s=\sqrt{\alpha'}$ y la constante de acoplamiento es $g_s$ en AdS$_5 \times S^5$ (el radio de curvatura del espacio AdS y de la esfera $L$ son iguales). Los parámetros libres de la teoría de campos ($g_{YM}$ y $N$) se relacionan con los parámetros libres de la teoría de supercuerdas ($g_s$ y $L/\sqrt{\alpha'}$ por medio de las ecuaciones
\begin{equation}
g_{YM}^2=2\pi g_s\,,\,\,\,\,2g_{YM}^2 N=\frac{L^4}{\alpha'^2\,}\,.
\end{equation}
La realización de esta dualidad es bastante peculiar, dado que permite relacionar una (posible) teoría cuántica de la gravedad (la teoría de supercuerdas $IIB$) con una teoría de campos que no contiene grados de libertad gravitacionales.

A pesar de que la forma más fuerte de la correspondencia AdS$_5$/CFT$_4$ presentada es muy interesante, es bastante complicado realizar cálculos específicos para valores genéricos de los parámetros libres. Por este motivo, es natural preguntarse si en ciertos límites existe una versión más débil de la correspondencia, con la cual hacer cálculos explícitos sea más factible. Dado que la teoría de cuerdas se entiende mejor en el régimen perturbativo, una propuesta es especificar la dualidad para el caso en $g_s \ll 1$, manteniendo $L/\sqrt{\alpha'}$ fijo. A primer orden no trivial en $g_s$, la parte AdS de la correspondencia queda reducida a una teoría clásica de cuerdas (en el sentido de que sólo intervienen diagramas tipo árbol). La longitud de la cuerda $l_s$ medida en unidades de $L$ se mantiene constante. En este límite (versión fuerte de la correspondencia), la teoría de campos involucrada en la correspondencia tiene $g_{YM}\ll 1$ y $\lambda\doteq g_{YM}^2 N$ (constante de 't Hooft) finito. En otras palabras, en la teoría de campos tenemos que tomar el límite de $N\longrightarrow \infty$ manteniendo $lambda$ fijo, lo que se conoce como límite de 't Hooft; esto corresponde al límite planar de la teoría de gauge.  En este régimen, la correspondencia AdS/CFT es una realización concreta de la idea de 't Hooft de que el límite planar de una teoría de campos cuántica es una teoría de cuerdas.

En el límite de 't Hooft, sólo hay un parámetro libre en cada lado de la correspondencia: el parámetro de 't Hooft $\lambda$ en la teoría de campos y $L/\sqrt{\alpha'}$ en la teoría de cuerdas. Estos dos parámetros se relacionan por $L^4/\alpha'^2=2\lambda$. Si estamos interesados en estudiar teorías de campos fuertemente interactuantes (para estudiar, por ejemplo, fenómenos no perturbativos), podemos tomar el límite $\lambda \longrightarrow \infty$ en la teoría de campos, lo que da $\sqrt{\alpha'}/L \longrightarrow 0$ en la teoría de cuerdas. En este caso, la longitud de la cuerda es muy pequeña comparada con el radio de curvatura, lo que indica que este es el límite de partícula puntual de la teoría $IIB$ (que está dado por la teoría de supergravedad $IIB$ en AdS$_5\times$S$^5$). Este límite de la correspondencia se conoce como forma débil de la dualidad AdS/CFT.

\section{Entropía holográfica de entrelazamiento}
CONTEXTO.

En este caso, la entropía de entrelazamiento en el borde de una teoría de campos se determina mediante un elegante cálculo geométrico en el dual gravitatorio \cite{rt1}. En particular, la entropía de entrelazamiento entre una región espacial $V$ y su complemento $\bar V$ en el borde se obtiene a partir de
 \be
S(V) = \frac{2\pi}{\lp^{d-1}}\ \mathrel{\mathop {\rm
ext}_{\scriptscriptstyle{\mv\sim V}} {}\!\!} \left[A(\mv)\right]
 \labell{define}
 \ee
donde hay que extremar el valor del área sobre todas las superficies $\mv$ en el bulk homólogas a $V$. Hemos adoptado la convención $\lp^{d-1}=8\pi G_\mt{N}$, donde $d$ es la dimensión espacio temporal del borde. Para casos estáticos, la ecuación \reef{define} se conoce como conjetura de Ryu-Takayanagi. En geometrías dependientes del tiempo, la ecuación \reef{define} se suele conocer como fórmula HRT (Hubeny, Rangamani, Takayanagi). En geometrías estáticas hay una coordenada tiempo $t$ natural y por simetría la superficie extremal siempre estará contenida en un corte del espacio tiempo a tiempo fijo. Si el tiempo está fijo, la superficie extremal es entonces la que tiene área mínimal, de modo que para el caso estático, la fórmula \reef{define} se reduce a encontrar la superficie que minimiza el funcional área. En cambio, para deformaciones en la dirección de $t$ las superficies extremales son las que tienen área máxima (dado que el área puede hacerse tan pequeña como desee haciendo que la superficie se aproxime a una superficie nula).

La prescripción \reef{define} ha pasado muchas pruebas de consistencia \cite{rt1,head,EEGB}; algunas de ellas se describen en la sección siguiente. Esta fórmula también ha sido derivada para el caso especial de regiones de entrelazamiento esféricas \cite{casini9} y, recientemente en \cite{aitor} la derivación ha sido extendida para el caso de superficies de entrelazamiento suaves generales.

La entropía de entrelazamiento es una medida de cómo se encuentra oganizada espacialmente la información cuántica en un estado cuántico. Para una teoría de campos general (no conforme), esperamos que la fórmula para calcular la entropía de entrelazamiento utilizando holografía sea extremadamente complicada. El hecho de que se simplifique a un sencillo cálculo geométrico en CFT holográficas revela una profunda característica de los sistemas fuertemente interactuantes; en el régimen de acoplamiento fuerte, la organización de la información cuántica se aproxima a un límite sencillo y universal. Cómo es que esto sucede y qué relación tiene con la geometría emergente es un importante problema abierto y de gran interés actual.

La teoría de la información cuántica provee también otras herramientas que permitirían refinar nuestro entendimiento sobre el entrelazamiento en teorías holográficas. Las entropías de Rényi, por ejemplo, son una familia infinita de medidas de entrelazamiento \cite{renyi0,karol} que proveen una descripción completa del espectro del operador densidad \cite{cala}. Desafortunadamente, el progreso en el entendimiento de las entropías de Rényi en teorías holográficas es aún bastante limitado \cite{head,twod,yale}. Una buena comprensión de las mismas se ha logrado para el caso de teorías conformes bidimensionales y también para el caso especial de regiones de entrelazamiento esféricas en cualquier dimensión \cite{yale}. Sin embargo, aún no se tiene una propuesta eficiente para calcular la entropías de Rényi en holografías para situaciones más generales. En el capítulo \ref{ch:hee} estudiamos otra medida de información, la entropía relativa (presentada en el capítulo anterior), en el contexto holográfico.

Volvamos a la fórmula \reef{define}. Es importante destacar que la misma da una contribución proporcional al área para la entropía, como se espera en general para el orden no trivial más importante. Además, es sencillo ver que si el estado es puro (esto se traduce en la ausencia de horizontes en el bulk), la entropía holográfica de una región y su complemento resultan idénticas, como se espera que suceda para la entropía de entrelazamiento.

A continuación, para entender un poco mejor cómo se utiliza la fórmula de Ryu-Takayanagi, presentamos un par de ejemplos en donde se calcula la entropía de entrelazamiento utilizando la ecuación \reef{define}, y que también sirven como indicadores de que esta prescripción sirve en efecto para calcular la entropía de entrelazamiento.

\subsection{Estado de vacío en 1+1 CFT}

Consideremos una teoría conforme en $1+1$ dimensiones y sea $V$ un intervalo de longitud $L$ dado por los puntos
\begin{equation}
x \in \left[-\frac{L}{2},\frac{L}{2}\right]\,.
\end{equation}
La geometría dual a esta teoría conforme es $AdS_3$, cuya métrica está dada por
\begin{equation}
ds^2=\frac{\ell^2}{z^2}\left(-dt^2+dx^2+dz^2\right)\,;
\end{equation}
$z$ es la dirección radial, y el la teoría de campos se encuentra en la superficie dada por $z=0$.

Consideremos el estado de vacío en la teoría de campos, para el cual queremos hallar la entropía. Este estado es estático, por lo que podemos tomar $t=0$. Una superficie extremal de codimensión $2$ en $AdS_3$ es unidimensional, es decir, es una geodésica. Luego, la fórmula \reef{define} nos indica que debemos hallar una geodésica espacial en la geometría
\begin{equation}
ds^2=\frac{\ell^2}{z^2}\left(dx^2+dz^2\right)\,,
\end{equation}
que conecte los puntos $P_1=\left(z_1,x_1\right)=\left(0,-\frac{L}{2}\right)$ y $P_2=\left(z_2,x_2\right)=\left(0,\frac{L}{2}\right)$. Sin embargo, cualquier geodésica que termine en $z=0$ va a tener longitud infinita, dado que $\int \frac{dz}{z}=+\infty$. Esto es el reflejo, en el dual gravitatorio, de las divergencias ultravioletas que presenta la entropía de entrelazamiento en teoría de campos. Para regular estas divergencias, introducimos un cutoff en $z=\epsilon$.

Parametrizando la curva en la forma $\left(z(\lambda),x(\lambda)\right)$, tenemos que la longitud (área) de la geodésica regularizada está dada por
\begin{equation}
A=\int ds = 2L \int_{\epsilon}^{z_{max}}\frac{dz}{z}\sqrt{x'(z)^2+1}\,.\label{aresp}
\end{equation}
Es sencillo mostrar que la geodésica está dada por una porción de círculo (casi un semicírculo)
\begin{equation}
x=\frac{L}{2}\cos\lambda\,,\,\,\,z=\frac{L}{2}\sin\lambda\,,\,\,\,\textrm{con}\,\,\lambda \in \left(\frac{\epsilon}{L},\pi-\frac{\epsilon}{L}\right)\,.
\end{equation}
Sustituyendo en \reef{aresp}, encontramos que el área de la superficie mínima es
\begin{equation}
A=2L\log\left(\frac{L}{\epsilon}\right)\,.
\end{equation}
\section{Propiedades de la entropía holográfica}

En esta sección, presentamos algunas de las propiedades que satisface la entropía holográfica de entrelazamiento. La validez de estas propiedades, que se sabe que satisface la entropía de entrelazamiento, constituye una prueba de consistencia para la fórmula \reef{define}.

\subsection{Subaditividad fuerte}

La propiedad de subaditividad fuerte fue presentada en la sección \ref{sec:propentro}; recordamos que para un sistema tripartito, la subaditividad fuerte dice que
\begin{equation}
S_{ABC}+S_B \leq S_{AB} + S_{BC}\,.\label{subanueva}
\end{equation}
La demostración de la validez de esta propiedad para la entropía holográfica es bastante sencilla para estados estáticos. En la figura \ref{holossa} se grafican las superficies minimales correspondientes a las regiones $ABC$, $B$, $AB$ y $BC$. Las dos superficies minimales homólogas a $AB$ y $BC$ pueden pensarse como dos superficies, en general no suaves, asociadas a superficies homólogas a las regiones $ABC$ y $B$, representadas en la figura en negro y azul, respectivamente. Como las superficies coloreadas en verde y rojo con las de área mínima homólogas a las regiones $ABC$ y $B$, respectivamente, deducimos que el área de la superficie roja es menor al de la superficie azul, y el área de la superficie negra es menor al de la verde. Sumando estas dos desigualdades y multiplicando globalmente por $\frac{2\pi}{\ell_p^{d-1}}$ obtenemos la propiedad de subaditividad fuerte \reef{subanueva}.
\begin{figure}[h]
\begin{center}
\includegraphics[width=13cm]{holossa.jpg}
\end{center}
\caption{\textbf{Subaditividad fuerte para la entropía holográfica}. Las curvas suaves homólogas a cada región, representan las superficies de área mínima. Las dos curvas asociadas a las superficies minimales homólogas a $AB$ y $BC$ pueden pensarse como dos curvas, en general no suaves, asociadas a superficies homólogas a las regiones $ABC$ y $B$ (representadas en negro y azul, respectivamente). Como las curvas en verde y rojo representan las superficies de área mínima homólogas a las regiones $ABC$ y $B$, respectivamente, se deduce que el área de la curva roja es menor a la de la curva azul, y el área de la curva negra es menor al de la verde. La suma de esas dos desigualdades demuestra la subaditividad fuerte para la entropía holográfica. } \label{holossa}
\end{figure}

Este argumento ha sido también extendido al caso de estados no estáticos \textbf{REFERENCIA}. Naturalmente, la demostración es un poco más complicada, dado que las superficies extremales no se encuentran necesariamente en un corte a tiempo constante.

\subsection{Entropía de Bekenstein-Hawking}



Introducir acá el capítulo siguiente, motivándolo como una prueba de consistencia más para la EHE (pero decir que los resultados que se van a mostrar dan cosas mucho más interesantes que eso).
